Controlling Latent Diffusion Using Latent CLIP

Instead of performing text-conditioned denoising in the image domain, latent diffusion models (LDMs) operate in latent space of a variational autoencoder (VAE), enabling more efficient processing at reduced computational costs. However, while the diffusion process has moved to the latent space, the contrastive language-image pre-training (CLIP) models, as used in many image processing tasks, still operate in pixel space. Doing so requires costly VAE-decoding of latent images before they can be processed. In this paper, we introduce Latent-CLIP, a CLIP model that operates directly in the latent space. We train Latent-CLIP on 2.7B pairs of latent images and descriptive texts, and show that it matches zero-shot classification performance of similarly sized CLIP models on both the ImageNet benchmark and a LDM-generated version of it, demonstrating its effectiveness in assessing both real and generated content. Furthermore, we construct Latent-CLIP rewards for reward-based noise optimization (ReNO) and show that they match the performance of their CLIP counterparts on GenEval and T2I-CompBench while cutting the cost of the total pipeline by 21%. Finally, we use Latent-CLIP to guide generation away from harmful content, achieving strong performance on the inappropriate image prompts (I2P) benchmark and a custom evaluation, without ever requiring the costly step of decoding intermediate images.

==> images/diffusion_algo.tex <==
\newcommand{\vardbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}
\newcommand{\defeq}{\coloneqq}
\newcommand{\grad}{\nabla}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\!\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\kl}[2]{D_{\mathrm{KL}}\!\left(#1 ~ \| ~ #2\right)}
\newcommand{\pdata}{{p_\mathrm{data}}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bxh}{\hat{\mathbf{x}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bnu}{{\boldsymbol{\nu}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
  \caption{Training} \label{alg:training}
  \small
  \begin{algorithmic}[1]
    \Repeat
      \State $\bx_0 \sim q(\bx_0)$
      \State $t \sim \mathrm{Uniform}(\{1, \dotsc, T\})$
      \State $\bepsilon\sim\mathcal{N}(\bzero,\bI)$
      \State Take gradient descent step on
      \Statex $\qquad \grad_\theta \left\| \bepsilon - \bepsilon_\theta(\sqrt{\bar\alpha_t} \bx_0 + \sqrt{1-\bar\alpha_t}\bepsilon, t) \right\|^2$
    \Until{converged}
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
  \caption{Sampling} \label{alg:sampling}
  \small
  \begin{algorithmic}[1]
    \vspace{.04in}
    \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
    \For{$t=T, \dotsc, 1$}
      \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz = \bzero$
      \State $\bx_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \bepsilon_\theta(\bx_t, t) \right) + \sigma_t \bz$
    \EndFor
    \State \textbf{return} $\bx_0$
    \vspace{.095in}
  \end{algorithmic}
\end{algorithm}
\end{minipage}
%\vspace{-1em}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/exp2-geneval.tex <==
\begin{table*}[h!]
  \centering
  \caption{Quantitative results on GenEval.} 
  \label{tab:geneval}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
  } % Added an extra column here
  \toprule
      \bfseries Model
    &{\bfseries Mean~$\uparrow$}
    &{\bfseries Single~$\uparrow$}
    &{\bfseries Two~$\uparrow$}
    &{\bfseries Counting~$\uparrow$}
    &{\bfseries Colors~$\uparrow$}
    &{\bfseries Pos.~$\uparrow$}
    &{\bfseries Color Attr.~$\uparrow$}
    &{\bfseries Aesthetic~$\uparrow$} \\
  \midrule
    \fixme{Base (SDXL-Turbo)}    & 0.54 & 0.99  & 0.66 & 0.45 & 0.85 & 0.09 & 0.20 & 5.39 \\ % Add values or placeholders (e.g., "--") for Aesthetic
    ReNO &  0.64 & 0.99  & 0.86 & 0.62 & 0.90 & 0.12 & 0.36 & 5.58 \\
  \midrule
    \bfseries CLIPScore \\
  \midrule
    \rowcolor{highlightcolor}
    \LatentViTxBE        & 0.6 & 0.98 & 0.78 & 0.53 & 0.89 & 0.12 & 0.32 & 5.40 \\
    \rowcolor{highlightcolor}
    \LatentViTxBF        & 0.62 & 0.99 & 0.82 & 0.6 & 0.9 & 0.14 & 0.3 & 5.40 \\
  %\midrule
    \CViTxBTTxLAION      & 0.61 & 0.99 & 0.82 & 0.59 & 0.89 & 0.11 & 0.27 & 5.43 \\
    \CViTxBTTxDataComp   & 0.59 & 0.99 & 0.78 & 0.55 & 0.88 & 0.11 & 0.23 & 5.43 \\
    \CViTxBSTxDataCompXL & 0.61 & 0.99 & 0.81 & 0.58 & 0.91 & 0.11 & 0.23 & 5.44 \\
    \CViTxGFTxLAION      & 0.62 & 1.00 & 0.82 & 0.6 & 0.92 & 0.11 & 0.27 & 5.44 \\
  \midrule
    \bfseries PickScore \\
  \midrule
    \rowcolor{highlightcolor}
    \LatentViTxBE        & 0.61 & 1.0 & 0.77 & 0.58 & 0.91 & 0.1 & 0.28 & 5.40 \\
    \rowcolor{highlightcolor}
    \LatentViTxBF        & 0.62 & 0.99 & 0.79 & 0.63 & 0.9 & 0.13 & 0.26 & 5.5 \\
  %\midrule
    \CViTxBTTxLAION      & 0.6 & 0.99 & 0.78 & 0.56 & 0.9 & 0.1 & 0.29 & 5.49 \\
    \CViTxBTTxDataComp   & 0.6 & 0.99 & 0.8 & 0.58 & 0.89 & 0.1 & 0.24 & 5.5 \\
    \CViTxBSTxDataCompXL & 0.6 & 1.0 & 0.75 & 0.58 & 0.89 & 0.1 & 0.26 & 5.52 \\
    \CViTxHFTxLAION      & 0.62 & 1.0 & 0.83 & 0.62 & 0.89 & 0.11 & 0.26 & 5.53 \\
  \bottomrule
\end{tabular}
%\vspace{-1em}
\end{table*}



==> tables/exp2-t2i.tex <==

\begin{table*} % [h!]
\centering
\caption{Quantitative results on T2I-CompBench.} 
\label{tab:t2icompbenchfull}
  \setlength{\tabcolsep}{1.5pt}
  \begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
    S[table-format=1.2]
  } % Added an extra column here
  \toprule
      \multirow{2}{*}{\bfseries Model}
    & \multicolumn{3}{c}{\bfseries Attribute Binding }
    & \multicolumn{2}{c}{\bfseries Object Relationship } \\ % Added Aesthetic column here
  \cmidrule(lr){2-4}\cmidrule(lr){5-6}
    & {\bfseries Color~$\uparrow$ } & {\bfseries Shape~$\uparrow$ } & { \bfseries Texture~$\uparrow$ }
    & {\bfseries Spatial~$\uparrow$ } & {\bfseries Non-Spatial$\uparrow$ }
    & {\bfseries Complex~$\uparrow$ }
    & {\bfseries Aesthetic~$\uparrow$ } \\
  \midrule
    \fixme{Base (SDXL-Turbo)}    & 0.62 & 0.44 & 0.60 & 0.24 & 0.31 & 0.42 & 5.51 \\ % Add values or placeholders (e.g., "--") for Aesthetic
    ReNO                 & 0.78 & 0.59 & 0.74 & 0.25 & 0.32 & 0.47 & 5.70 \\
  \midrule
    {\bfseries CLIPScore } \\
  \midrule
    \rowcolor{highlightcolor}
    {\LatentViTxBE}       & 0.68 & 0.54 & 0.69 & 0.25 & 0.32 & 0.44 & 5.54 \\
    \rowcolor{highlightcolor}
    {\LatentViTxBF}      & 0.69 & 0.54 & 0.70 & 0.24 & 0.32 & 0.44 & 5.55 \\
  %\midrule
    \CViTxBTTxLAION      & 0.69 & 0.54 & 0.68 & 0.23 & 0.32 & 0.44 & 5.56 \\
    \CViTxBTTxDataComp   & 0.67 & 0.53 & 0.68 & 0.24 & 0.32 & 0.43 & 5.56 \\
    \CViTxBSTxDataCompXL & 0.67 & 0.53 & 0.68 & 0.24 & 0.32 & 0.45 & 5.55 \\
    \CViTxGFTxLAION      & 0.69 & 0.54 & 0.69 & 0.23 & 0.32 & 0.44 & 5.56 \\
  \midrule
    {\bfseries PickScore } \\
  \midrule
    \rowcolor{highlightcolor}
    {\LatentViTxBE}      & 0.65 & 0.51 & 0.65 & 0.25 & 0.31 & 0.45 & 5.60 \\
    \rowcolor{highlightcolor}
    {\LatentViTxBF}      & 0.68 & 0.52 & 0.65 & 0.25 & 0.31 & 0.44 & 5.67 \\
  %\midrule
    \CViTxBTTxLAION      & 0.65 & 0.51 & 0.65 & 0.24 & 0.31 & 0.42 & 5.66 \\
    \CViTxBTTxDataComp   & 0.66 & 0.51 & 0.66 & 0.24 & 0.31 & 0.42 & 5.66 \\
    \CViTxBSTxDataCompXL & 0.65 & 0.50 & 0.65 & 0.26 & 0.31 & 0.43 & 5.67 \\
    \CViTxHFTxLAION      & 0.66 & 0.52 & 0.66 & 0.24 & 0.31 & 0.43 & 5.70 \\
  \bottomrule
\end{tabular}
%\vspace{-1em}
\end{table*}




%fürn anhang
\iffalse
\midrule
{\textbf{CLIPScore}} \\
\midrule

\rowcolor{lavender}
{Latent-ViT-B-8-512} & 0.6823 & 0.5372 & 0.6867 & 0.25 & 0.3176 & 0.4447 & 5.542 \\
\rowcolor{lavender}
{Latent-ViT-B-4-512-plus} & 0.6887 & 0.5428 & 0.6996 & 0.2435 & 0.3173 & 0.445 & 5.546 \\
%\midrule
CLIP-ViT-B-32-laion2B-s34B-b79K & 0.6917 & 0.5407 & 0.6792 & 0.2338 & 0.3202 & 0.4413 & 5.561 \\
CLIP-ViT-B-32-256x256-DataComp-s34B-b86K & 0.6736 & 0.533 & 0.6847 & 0.2403 & 0.3166 & 0.4284 & 5.557 \\
CLIP-ViT-B-16-DataComp.XL-s13B-b90K & 0.6741 & 0.534 & 0.6844 & 0.2395 & 0.316 & 0.4466 & 5.553 \\
CLIP-ViT-g-14-laion2B-s34B-b88K  & 0.6888 & 0.5355 & 0.6871 & 0.2337 & 0.3158 & 0.4419 & 5.556 \\

\midrule
{\textbf{PickScore}} \\
\midrule

\rowcolor{lavender}
{Latent-ViT-B-8-512} & 0.6532 & 0.507 & 0.6459 & 0.2541 & 0.3142 & 0.4456 & 5.598 \\
\rowcolor{lavender}
{Latent-ViT-B-4-512-plus} & 0.6825 & 0.5177 & 0.6538 & 0.2539 & 0.3143 & 0.4351 & 5.667 \\
%\midrule
CLIP-ViT-B-32-laion2B-s34B-b79K & 0.6534 & 0.5079 & 0.6469 & 0.2354 & 0.3121 & 0.4223 & 5.662 \\
CLIP-ViT-B-32-256x256-DataComp-s34B-b86K & 0.6645 & 0.5122 & 0.6574 & 0.2384 & 0.3131 & 0.4192 & 5.664 \\
CLIP-ViT-B-16-DataComp.XL-s13B-b90K & 0.6508 & 0.5001 & 0.6546 & 0.2601 & 0.3124 & 0.4313 & 5.671 \\
CLIP-ViT-H-14-laion2B-s32B-b79K  & 0.6588 & 0.5193 & 0.6593 & 0.2436 & 0.3116 & 0.4291 & 5.696 \\

\fi

==> tables/exp2-time-gain.tex <==
\begin{table}[h!]
  \caption{Computation times per iteration and total over 50 steps for different reward models in ReNO.}
  \centering
  \label{tab:timing_results}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=2.2, round-precision=2]
  }
  \toprule
    \bfseries Model & {\bfseries Per Iter.} & {\bfseries Total} \\
  \midrule
    \fixme{SDXL-Turbo (No VAE-decoder)} & 0.16 & 5.75 \\ % & 0.115 & 5.750 \\
    ReNO                 & 0.45 & 22.51 \\ % & 0.450 & 22.509 \\
  \midrule
    \LatentViTxBE        & 0.18 & 9.11 \\ % & 0.182 & 9.112 \\
    \LatentViTxBF        & 0.18 & 9.01 \\ % & 0.180 & 9.006 \\
  \midrule
    \CViTxBTTxLAION      & 0.23 & 11.59 \\ % & 0.232 & 11.586 \\
    \CViTxBSTPxLAION     & 0.24 & 11.78 \\ % & 0.236 & 11.784 \\
    \CViTxBSTxLAION      & 0.24 & 11.87 \\ % & 0.237 & 11.869 \\
    \CViTxBTTxDataComp   & 0.23 & 11.64 \\ % & 0.233 & 11.638 \\
    \CViTxBSTxDataCompXL & 0.23 & 11.70 \\ % & 0.234 & 11.699 \\
    \CViTxLFTxLAION      & 0.25 & 12.32 \\ % & 0.246 & 12.324 \\
    \CViTxHFTxLAION      & 0.27 & 13.27 \\ % & 0.265 & 13.271 \\
    \CViTxGFTxLAION      & 0.27 & 13.50 \\ % & 0.270 & 13.503 \\
  \bottomrule
\end{tabular}
\end{table}


\iffalse
Latent-ViT-B-8-512
Latent-ViT-B-4-512-plus

CLIP-ViT-B-32-laion2B-s34B-b79K
CLIP-ViT-B-16-plus-240-laion400m-e32
CLIP-ViT-B-16-laion2B-s34B-b88K
CLIP-ViT-B-32-256x256-DataComp-s34B-b86K
CLIP-ViT-B-16-DataComp.XL-s13B-b90K
CLIP-ViT-L-14-laion2B-s32B-b82K
CLIP-ViT-H-14-laion2B-s32B-b79K
CLIP-ViT-g-14-laion2B-s34B-b88K
\fi

==> tables/exp4-initial-bias.tex <==
\begin{table}[h!]
\centering
\caption{Probability of generating explicit content using SDXL Turbo.}
\label{tab:exp4-initial}
%\resizebox{\columnwidth}{!}{ 
\begin{tabular}{lc}
\toprule
\textbf{Prompt} & \textbf{Probability} \\
\midrule
``u.s. american body''   & 0.01 \\
``german body''          & 0.03 \\
``nigerian body''        & 0.20 \\
``european body''        & 0.21 \\
``japanese body''        & 0.65 \\
``asian body''           & 0.75 \\

\bottomrule
\end{tabular}

\end{table}


==> tables/interpolate.tex <==
\newcommand{\xa}{\makebox[0pt][l]{$^a$}}
\newcommand{\xb}{\makebox[0pt][l]{$^b$}}
%$^\dagger$

\begin{table}[htbp]
  \caption{Classification performance of Latent CLIP and traditional CLIP models across workflows and interpolation methods. (1) indicates directly using the interpolated latents, while (2) refers to latents obtained by resizing the generated images and then decoding them back into latent space.}
  \label{tab:interpolation_comparison_table}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lccccc}
    \toprule
    \textbf{Model} & \textbf{Interpolation} & \multicolumn{2}{c}{\textbf{Basic Workflow}} & \multicolumn{2}{c}{\textbf{Advanced Workflow}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    & & \textbf{Top-1} & \textbf{Top-5} & \textbf{Top-1} & \textbf{Top-5} \\
    \midrule
    \multirow{3}{*}{(1) Latent-ViT-B-8-512} 
        & bilinear & 50.3 & 75.6  & 44.7 & 70.2 \\
        & bicubic & 49.6 & 74.9  & 36.0 & 60.6 \\
        & nearest & 55.9 & 80.5  & 38.9 & 64.3 \\
    \cmidrule(lr){2-6} % Adds a line from the second to the last column
    
    %\midrule
    \multirow{3}{*}{(1) Latent-ViT-B-4-512-plus}
        & bilinear & 43.6 & 68.5  & 44.9 & 70.4 \\
        & bicubic  & 50.3 & 75.9  & 42.0 & 67.1 \\
        & nearest & 62.9 & 85.8  & 49.2 & 75.1 \\
        
    \midrule
    \midrule 
    
    % Regular midrule for separation between the two sections
    \multirow{1}{*}{CLIP-ViT-B-32-laion2B-s34B-b79K} 
        & - & 79.8 & 95.2  & 73.5 & 92.9 \\
    %\cmidrule(lr){2-6} % Line from the second to the last column for the last two models
    
    \multirow{1}{*}{CLIP-ViT-B-16-DataComp.XL-s13B-b90K} 
        & - & 83.1 & 96.5  & 78.2 & 94.8 \\
        
    \multirow{1}{*}{CLIP-ViT-g-14-laion2B-s34B-b88K} 
        & - & 84.7 & 96.9  & 81.4 & 96.0 \\
        
    \midrule
    \midrule  % Regular midrule for separation between the two sections
    
    \multirow{1}{*}{(2) Latent-ViT-B-8-512} 
        & - & 79.9 & 95.6  & 74.1 & 93.2 \\
    %\cmidrule(lr){2-6} % Line from the second to the last column for the last two models
    \multirow{1}{*}{(2) Latent-ViT-B-4-512-plus} 
        & - & 82.6 & 96.4  & 78.3 & 94.8 \\
        
    \bottomrule
  \end{tabular}
  }
\end{table}


==> tables/xlturboworkflow.tex <==
%$^\dagger$

\begin{table}[htbp]
  \caption{Classification performance of Latent CLIP and traditional CLIP models on the evaluation dataset generated by the our SDXL Turbo workflow. (1) indicates directly using the generated latents, while (2) refers to latents obtained by resizing the generated images and then decoding them back into latent space.}
  \label{tab:turbo_comparison_table}
  \centering
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{
    l
    S[table-format=2.1]
    S[table-format=2.1]
  }
  \toprule
    \multirow{2}{*}{\bfseries Model} & \multicolumn{2}{c}{\bfseries \textcolor{red}{Accuracy}}  \\
                                    \cmidrule(lr){2-3} 
                                     & {\bfseries Top-1 } & {\bfseries Top-5}  \\
  \midrule
    \rowcolor{highlightcolor}
    (1) \LatentViTxBF    & 84.6 & 98.0 \\
    \rowcolor{highlightcolor}
    (2) \LatentViTxBF    & 84.6 & 98.0 \\
    \CViTxBSTPxLAION     & 82.8 & 97.6 \\
    \CViTxBSTxLAION      & 83.8 & 97.7 \\
    \CViTxBSTxDataCompXL & 85.1 & 98.0 \\
    \CViTxLFTxLAION      & 86.0 & 98.2 \\
    \CViTxHFTxLAION      & 87.0 & 98.5 \\
    \CViTxGFTxLAION      & 86.8 & 98.4 \\
  \midrule
    \rowcolor{highlightcolor}
    (1) \LatentViTxBE    & 81.7 & 97.3 \\
    \rowcolor{highlightcolor}
    (2) \LatentViTxBE    & 82.0 & 97.3 \\
    \CViTxBTTxLAION      & 82.1 & 97.2 \\
    \CViTxBTTxDataComp   & 84.5 & 98.0 \\
        
        
  \bottomrule
  \end{tabular}
\end{table}

